PATHS: A Hierarchical Transformer for Efficient Whole Slide Image Analysis

Computational analysis of whole slide images (WSIs) has seen significant research progress in recent years, with applications ranging across important diagnostic and prognostic tasks such as survival or cancer subtype prediction. Many state-of-the-art models process the entire slide - which may be as large as $150,000 \times 150,000$ pixels - as a bag of many patches, the size of which necessitates computationally cheap feature aggregation methods. However, a large proportion of these patches are uninformative, such as those containing only healthy or adipose tissue, adding significant noise and size to the bag. We propose Pathology Transformer with Hierarchical Selection (PATHS), a novel top-down method for hierarchical weakly supervised representation learning on slide-level tasks in computational pathology. PATHS is inspired by the cross-magnification manner in which a human pathologist examines a slide, recursively filtering patches at each magnification level to a small subset relevant to the diagnosis. Our method overcomes the complications of processing the entire slide, enabling quadratic self-attention and providing a simple interpretable measure of region importance. We apply PATHS to five datasets of The Cancer Genome Atlas (TCGA), and achieve superior performance on slide-level prediction tasks when compared to previous methods, despite processing only a small proportion of the slide.

==> sec/scratch <==
Old algorithms which werent very good:

\Procedure{Process}{$\Xms{m_i}, \C$}
    \State $F_X \longleftarrow \imenc(\Xms{m_i})$ \label{line:patch_features} % \Comment{Compute patch features}
    \State $\alpha^i \longleftarrow \textsc{Imp}_i(F_X)$
    \State $F_X \longleftarrow F_X \odot \alpha^i$
    \State $F_L \longleftarrow \textsc{LocalAgg}_i(F_X, \C)$ \label{line:local_agg} %\Comment{Compute local features}
    \State $F_G \longleftarrow \textsc{GlobalAgg}_i(F_L)$ \label{line:global_agg} %\Comment{Compute slide-level features}
    %\State $\alpha \longleftarrow \textsc{Combine}(\alpha_L, \alpha_G)$ \label{line:combine_imp}
    \State \textbf{return} $(F_G, F_X, \alpha^i)$ \label{line:return}



NTS: Should probably treat X^m as the patch embeds rather than the raw patches, ie X^m new = I(X^m old). I very rarely want to talk about the patches themselves (maybe new notation for this such as P^m)



Old ablation tables:
%% OLD OLD ABLATION TABLE (BRCA only)
% \begin{table*}
%     \centering
%     \advance\leftskip-1cm
%     \advance\rightskip-1cm
%     % \resizebox{\textwidth}{!}{%
%         \caption[Context Ablation]{Ablation on various features of the architecture, assessing c-index on the IDC subtype when removing different features of our method.}
%     \begin{tabular}{c|cccc|c}
%          \toprule
%          \multirow{2}{*}{Model} & \multicolumn{4}{|c|}{\bf w/o} & \\
%         & Slide context & Hierarchical context & Attentional sampling & Pre-training of $\imenc$ & \name \\
%          \midrule
%          C-index & $0.597 \pm 0.050$ & $0.604 \pm 0.034$ & $0.604 \pm 0.040$ & $0.599 \pm 0.054$ & $\bf 0.625 \pm 0.033$\\
%          \bottomrule
%     \end{tabular}
%     % }

%     \label{tab:ablation_without_stuff}
% \end{table*}

% Old ablation table (when random + removing hierarchical context improved performance)
% \begin{table*}
%     \centering
%     \advance\leftskip-1cm
%     \advance\rightskip-1cm
%     % \resizebox{\textwidth}{!}{%
%         \caption[Ablation]{Ablation study: we measure model performance (c-index) with different components of our architecture individually removed.}
%     \begin{tabular}{c|ccc|c}
%          \toprule
%          \multirow{2}{*}{Model} & \multicolumn{3}{|c|}{\bf w/o} & \\
%         & Slide context & Hierarchical context & Attentional sampling & \name \\
%          \midrule
%          IDC & $0.597 \pm 0.050$ & $0.604 \pm 0.034$ & $0.604 \pm 0.040$ & $0.625 \pm 0.033$\\
%          CRC & $0.596 \pm 0.127$ & $0.690 \pm 0.075$ & $0.635 \pm 0.085$ & $0.608 \pm 0.086$\\
%          CCRCC & $0.637 \pm 0.039$ & $0.649 \pm 0.059$ & $0.655 \pm 0.045$ & $0.652 \pm 0.032$\\
%          PRCC & $0.653 \pm 0.038$ & $0.710 \pm 0.053$ & $0.748 \pm 0.038$ & $0.709 \pm 0.075$ \\
%          LUAD & $0.504 \pm 0.090$ & $0.553 \pm 0.079$ & $0.570 \pm 0.060$ & $0.564 \pm 0.058$ \\
%          \midrule
%          Mean & 0.597 & 0.641 & 0.642 & 0.632 \\
%          \bottomrule
%     \end{tabular}
%     % }

%     \label{tab:ablation_without_stuff}
% \end{table*}







REMOVED ABLATION NONSENSE

% To investigate the significance of our two forms of context (slide and patch-level), - and our attentive method for selecting patches, we run experiments with each component removed from the architecture. To remove slide-level context we set the slide-level feature $\Cs(i)$ to an empty list, so predictions at each stage $i$ use only patches at magnification $m^i$ and patch-level context. To remove hierarchical context, we drop the local aggregation step, using global aggregation only and therefore ignoring patch-level (hierarchical) context.

% remove the concatenation step, leaving only patch-level context. To remove hierarchical context, we drop the local aggregation step, using global aggregation only and therefore ignoring patch-level context. Finally, to remove attentive sampling (the selection of patches based on importance values $\imp$), we instead sample randomly, but still in a hierarchical manner; this is equivalent to randomising the importance values $\imp$ before carrying out the $\filter$ operation, so this method still benefits from both forms of context.







% Aux loss term no longer needed
% To prevent the model from assigning identical importance to all patches, we incorporate an auxiliary loss term encouraging high standard deviation in $\imp^i$,
% \[
% \imploss = -\sqrt{\mathbb{V}[\imp^i_{u,v}]}
% \]
% % weighted by a hyperparameter $$
% where $(u,v)$ are sampled uniformly from
% % where $D=\text{dom}(\Xms{m_i})$ is
% the set of patch locations in the selected subset $\Xms{m_i}$.







% Aggregation is split into two stages: local aggregation, conditioned on hierarchical context, and global aggregation. This is necessitated by the \textit{patch-dependent} nature of the hierarchical context, preventing a single global aggregation step. The two-stage aggregation approach resembles the restricted attention windows of the Swin transformer, and similarly reduces computational requirements by passing smaller sequence lengths to the self-attention modules~\cite{Swin}.

% Local aggregation no longer used...
% \textbf{Local Aggregation}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{local_agg.pdf}
%     \caption{Architecture of the local aggregator. Patches are grouped into $\magf \times \magf$ `neighbourhoods' ($\magf=2$ shown), then aggregated using a transformer. Cross-attention is applied to the hierarchical context of the neighbourhood via an encoder-decoder architecture. The resulting local features are globally aggregated into a slide-level feature.}
%     \label{fig:local_agg}
% \end{figure}
% \Cref{fig:local_agg} illustrates the architecture of the local aggregator. A patch at position $(u, v)$ shares an immediate parent in the hierarchy, and therefore hierarchical context, with a `neighbourhood' of $\magf^2$ surrounding patches. The first step of local aggregation is therefore to group patches into such neighbourhoods, which are each aggregated via a transformer encoder-decoder architecture; the (shared) hierarchical context is passed into the encoder, and the patch embeddings of the neighbourhood into the decoder, producing a single hierarchy-aware local feature. A single `special token' is passed to the decoder to produce the aggregated feature, as in the vision transformer \cite{ViT}.



% TODO: Big O bounds for num patches with my method vs full
%  rewrite this paragraph to be in terms of magnification m, slide height width h, w as that makes more sense. 
% Due to the bound \Cref{eq:patch_bound}, the number of patches extracted per slide by \name{} is bounded by $\O(\magf^2 \npatch \nmag)$, growing linearly in the depth of the hierarchy. The total number of patches at magnification $m$ is proportional to $m^2$, and as $m_\nmag = M^\nmag m_1$, the total number of patches $\O(M^(\nmag )$

